GAN2GAN: Generative Noise Learning for Blind Denoising with Single Noisy Images

We tackle a challenging blind image denoising problem, in which only single distinct noisy images are available for training a denoiser, and no information about noise is known, except for it being zero-mean, additive, and independent of the clean image. In such a setting, which often occurs in practice, it is not possible to train a denoiser with the standard discriminative training or with the recently developed Noise2Noise (N2N) training; the former requires the underlying clean image for the given noisy image, and the latter requires two independently realized noisy image pair for a clean image. To that end, we propose GAN2GAN (Generated-Artificial-Noise to Generated-Artificial-Noise) method that first learns a generative model that can 1) simulate the noise in the given noisy images and 2) generate a rough, noisy estimates of the clean images, then 3) iteratively trains a denoiser with subsequently synthesized noisy image pairs (as in N2N), obtained from the generative model. In results, we show the denoiser trained with our GAN2GAN achieves an impressive denoising performance on both synthetic and real-world datasets for the blind denoising setting; it almost approaches the performance of the standard discriminatively-trained or N2N-trained models that have more information than ours, and it significantly outperforms the recent baseline for the same setting, \textit{e.g.}, Noise2Void, and a more conventional yet strong one, BM3D. The official code of our method is available at https://github.com/csm9493/GAN2GAN.

==> math_commands.tex <==
\pdfoutput=1
%%%%% NEW MATH DEFINITIONS %%%%%

\usepackage{amsmath,amsfonts,bm}

% Mark sections of captions for referring to divisions of figures
\newcommand{\figleft}{{\em (Left)}}
\newcommand{\figcenter}{{\em (Center)}}
\newcommand{\figright}{{\em (Right)}}
\newcommand{\figtop}{{\em (Top)}}
\newcommand{\figbottom}{{\em (Bottom)}}
\newcommand{\captiona}{{\em (a)}}
\newcommand{\captionb}{{\em (b)}}
\newcommand{\captionc}{{\em (c)}}
\newcommand{\captiond}{{\em (d)}}

% Highlight a newly defined term
\newcommand{\newterm}[1]{{\bf #1}}


% Figure reference, lower-case.
\def\figref#1{figure~\ref{#1}}
% Figure reference, capital. For start of sentence
\def\Figref#1{Figure~\ref{#1}}
\def\twofigref#1#2{figures \ref{#1} and \ref{#2}}
\def\quadfigref#1#2#3#4{figures \ref{#1}, \ref{#2}, \ref{#3} and \ref{#4}}
% Section reference, lower-case.
\def\secref#1{section~\ref{#1}}
% Section reference, capital.
\def\Secref#1{Section~\ref{#1}}
% Reference to two sections.
\def\twosecrefs#1#2{sections \ref{#1} and \ref{#2}}
% Reference to three sections.
\def\secrefs#1#2#3{sections \ref{#1}, \ref{#2} and \ref{#3}}
% Reference to an equation, lower-case.
\def\eqref#1{equation~\ref{#1}}
% Reference to an equation, upper case
\def\Eqref#1{Equation~\ref{#1}}
% A raw reference to an equation---avoid using if possible
\def\plaineqref#1{\ref{#1}}
% Reference to a chapter, lower-case.
\def\chapref#1{chapter~\ref{#1}}
% Reference to an equation, upper case.
\def\Chapref#1{Chapter~\ref{#1}}
% Reference to a range of chapters
\def\rangechapref#1#2{chapters\ref{#1}--\ref{#2}}
% Reference to an algorithm, lower-case.
\def\algref#1{algorithm~\ref{#1}}
% Reference to an algorithm, upper case.
\def\Algref#1{Algorithm~\ref{#1}}
\def\twoalgref#1#2{algorithms \ref{#1} and \ref{#2}}
\def\Twoalgref#1#2{Algorithms \ref{#1} and \ref{#2}}
% Reference to a part, lower case
\def\partref#1{part~\ref{#1}}
% Reference to a part, upper case
\def\Partref#1{Part~\ref{#1}}
\def\twopartref#1#2{parts \ref{#1} and \ref{#2}}

\def\ceil#1{\lceil #1 \rceil}
\def\floor#1{\lfloor #1 \rfloor}
\def\1{\bm{1}}
\newcommand{\train}{\mathcal{D}}
\newcommand{\valid}{\mathcal{D_{\mathrm{valid}}}}
\newcommand{\test}{\mathcal{D_{\mathrm{test}}}}

\def\eps{{\epsilon}}


% Random variables
\def\reta{{\textnormal{$\eta$}}}
\def\ra{{\textnormal{a}}}
\def\rb{{\textnormal{b}}}
\def\rc{{\textnormal{c}}}
\def\rd{{\textnormal{d}}}
\def\re{{\textnormal{e}}}
\def\rf{{\textnormal{f}}}
\def\rg{{\textnormal{g}}}
\def\rh{{\textnormal{h}}}
\def\ri{{\textnormal{i}}}
\def\rj{{\textnormal{j}}}
\def\rk{{\textnormal{k}}}
\def\rl{{\textnormal{l}}}
% rm is already a command, just don't name any random variables m
\def\rn{{\textnormal{n}}}
\def\ro{{\textnormal{o}}}
\def\rp{{\textnormal{p}}}
\def\rq{{\textnormal{q}}}
\def\rr{{\textnormal{r}}}
\def\rs{{\textnormal{s}}}
\def\rt{{\textnormal{t}}}
\def\ru{{\textnormal{u}}}
\def\rv{{\textnormal{v}}}
\def\rw{{\textnormal{w}}}
\def\rx{{\textnormal{x}}}
\def\ry{{\textnormal{y}}}
\def\rz{{\textnormal{z}}}

% Random vectors
\def\rvepsilon{{\mathbf{\epsilon}}}
\def\rvtheta{{\mathbf{\theta}}}
\def\rva{{\mathbf{a}}}
\def\rvb{{\mathbf{b}}}
\def\rvc{{\mathbf{c}}}
\def\rvd{{\mathbf{d}}}
\def\rve{{\mathbf{e}}}
\def\rvf{{\mathbf{f}}}
\def\rvg{{\mathbf{g}}}
\def\rvh{{\mathbf{h}}}
\def\rvu{{\mathbf{i}}}
\def\rvj{{\mathbf{j}}}
\def\rvk{{\mathbf{k}}}
\def\rvl{{\mathbf{l}}}
\def\rvm{{\mathbf{m}}}
\def\rvn{{\mathbf{n}}}
\def\rvo{{\mathbf{o}}}
\def\rvp{{\mathbf{p}}}
\def\rvq{{\mathbf{q}}}
\def\rvr{{\mathbf{r}}}
\def\rvs{{\mathbf{s}}}
\def\rvt{{\mathbf{t}}}
\def\rvu{{\mathbf{u}}}
\def\rvv{{\mathbf{v}}}
\def\rvw{{\mathbf{w}}}
\def\rvx{{\mathbf{x}}}
\def\rvy{{\mathbf{y}}}
\def\rvz{{\mathbf{z}}}

% Elements of random vectors
\def\erva{{\textnormal{a}}}
\def\ervb{{\textnormal{b}}}
\def\ervc{{\textnormal{c}}}
\def\ervd{{\textnormal{d}}}
\def\erve{{\textnormal{e}}}
\def\ervf{{\textnormal{f}}}
\def\ervg{{\textnormal{g}}}
\def\ervh{{\textnormal{h}}}
\def\ervi{{\textnormal{i}}}
\def\ervj{{\textnormal{j}}}
\def\ervk{{\textnormal{k}}}
\def\ervl{{\textnormal{l}}}
\def\ervm{{\textnormal{m}}}
\def\ervn{{\textnormal{n}}}
\def\ervo{{\textnormal{o}}}
\def\ervp{{\textnormal{p}}}
\def\ervq{{\textnormal{q}}}
\def\ervr{{\textnormal{r}}}
\def\ervs{{\textnormal{s}}}
\def\ervt{{\textnormal{t}}}
\def\ervu{{\textnormal{u}}}
\def\ervv{{\textnormal{v}}}
\def\ervw{{\textnormal{w}}}
\def\ervx{{\textnormal{x}}}
\def\ervy{{\textnormal{y}}}
\def\ervz{{\textnormal{z}}}

% Random matrices
\def\rmA{{\mathbf{A}}}
\def\rmB{{\mathbf{B}}}
\def\rmC{{\mathbf{C}}}
\def\rmD{{\mathbf{D}}}
\def\rmE{{\mathbf{E}}}
\def\rmF{{\mathbf{F}}}
\def\rmG{{\mathbf{G}}}
\def\rmH{{\mathbf{H}}}
\def\rmI{{\mathbf{I}}}
\def\rmJ{{\mathbf{J}}}
\def\rmK{{\mathbf{K}}}
\def\rmL{{\mathbf{L}}}
\def\rmM{{\mathbf{M}}}
\def\rmN{{\mathbf{N}}}
\def\rmO{{\mathbf{O}}}
\def\rmP{{\mathbf{P}}}
\def\rmQ{{\mathbf{Q}}}
\def\rmR{{\mathbf{R}}}
\def\rmS{{\mathbf{S}}}
\def\rmT{{\mathbf{T}}}
\def\rmU{{\mathbf{U}}}
\def\rmV{{\mathbf{V}}}
\def\rmW{{\mathbf{W}}}
\def\rmX{{\mathbf{X}}}
\def\rmY{{\mathbf{Y}}}
\def\rmZ{{\mathbf{Z}}}

% Elements of random matrices
\def\ermA{{\textnormal{A}}}
\def\ermB{{\textnormal{B}}}
\def\ermC{{\textnormal{C}}}
\def\ermD{{\textnormal{D}}}
\def\ermE{{\textnormal{E}}}
\def\ermF{{\textnormal{F}}}
\def\ermG{{\textnormal{G}}}
\def\ermH{{\textnormal{H}}}
\def\ermI{{\textnormal{I}}}
\def\ermJ{{\textnormal{J}}}
\def\ermK{{\textnormal{K}}}
\def\ermL{{\textnormal{L}}}
\def\ermM{{\textnormal{M}}}
\def\ermN{{\textnormal{N}}}
\def\ermO{{\textnormal{O}}}
\def\ermP{{\textnormal{P}}}
\def\ermQ{{\textnormal{Q}}}
\def\ermR{{\textnormal{R}}}
\def\ermS{{\textnormal{S}}}
\def\ermT{{\textnormal{T}}}
\def\ermU{{\textnormal{U}}}
\def\ermV{{\textnormal{V}}}
\def\ermW{{\textnormal{W}}}
\def\ermX{{\textnormal{X}}}
\def\ermY{{\textnormal{Y}}}
\def\ermZ{{\textnormal{Z}}}

% Vectors
\def\vzero{{\bm{0}}}
\def\vone{{\bm{1}}}
\def\vmu{{\bm{\mu}}}
\def\vtheta{{\bm{\theta}}}
\def\va{{\bm{a}}}
\def\vb{{\bm{b}}}
\def\vc{{\bm{c}}}
\def\vd{{\bm{d}}}
\def\ve{{\bm{e}}}
\def\vf{{\bm{f}}}
\def\vg{{\bm{g}}}
\def\vh{{\bm{h}}}
\def\vi{{\bm{i}}}
\def\vj{{\bm{j}}}
\def\vk{{\bm{k}}}
\def\vl{{\bm{l}}}
\def\vm{{\bm{m}}}
\def\vn{{\bm{n}}}
\def\vo{{\bm{o}}}
\def\vp{{\bm{p}}}
\def\vq{{\bm{q}}}
\def\vr{{\bm{r}}}
\def\vs{{\bm{s}}}
\def\vt{{\bm{t}}}
\def\vu{{\bm{u}}}
\def\vv{{\bm{v}}}
\def\vw{{\bm{w}}}
\def\vx{{\bm{x}}}
\def\vy{{\bm{y}}}
\def\vz{{\bm{z}}}

% Elements of vectors
\def\evalpha{{\alpha}}
\def\evbeta{{\beta}}
\def\evepsilon{{\epsilon}}
\def\evlambda{{\lambda}}
\def\evomega{{\omega}}
\def\evmu{{\mu}}
\def\evpsi{{\psi}}
\def\evsigma{{\sigma}}
\def\evtheta{{\theta}}
\def\eva{{a}}
\def\evb{{b}}
\def\evc{{c}}
\def\evd{{d}}
\def\eve{{e}}
\def\evf{{f}}
\def\evg{{g}}
\def\evh{{h}}
\def\evi{{i}}
\def\evj{{j}}
\def\evk{{k}}
\def\evl{{l}}
\def\evm{{m}}
\def\evn{{n}}
\def\evo{{o}}
\def\evp{{p}}
\def\evq{{q}}
\def\evr{{r}}
\def\evs{{s}}
\def\evt{{t}}
\def\evu{{u}}
\def\evv{{v}}
\def\evw{{w}}
\def\evx{{x}}
\def\evy{{y}}
\def\evz{{z}}

% Matrix
\def\mA{{\bm{A}}}
\def\mB{{\bm{B}}}
\def\mC{{\bm{C}}}
\def\mD{{\bm{D}}}
\def\mE{{\bm{E}}}
\def\mF{{\bm{F}}}
\def\mG{{\bm{G}}}
\def\mH{{\bm{H}}}
\def\mI{{\bm{I}}}
\def\mJ{{\bm{J}}}
\def\mK{{\bm{K}}}
\def\mL{{\bm{L}}}
\def\mM{{\bm{M}}}
\def\mN{{\bm{N}}}
\def\mO{{\bm{O}}}
\def\mP{{\bm{P}}}
\def\mQ{{\bm{Q}}}
\def\mR{{\bm{R}}}
\def\mS{{\bm{S}}}
\def\mT{{\bm{T}}}
\def\mU{{\bm{U}}}
\def\mV{{\bm{V}}}
\def\mW{{\bm{W}}}
\def\mX{{\bm{X}}}
\def\mY{{\bm{Y}}}
\def\mZ{{\bm{Z}}}
\def\mBeta{{\bm{\beta}}}
\def\mPhi{{\bm{\Phi}}}
\def\mLambda{{\bm{\Lambda}}}
\def\mSigma{{\bm{\Sigma}}}

% Tensor
\DeclareMathAlphabet{\mathsfit}{\encodingdefault}{\sfdefault}{m}{sl}
\SetMathAlphabet{\mathsfit}{bold}{\encodingdefault}{\sfdefault}{bx}{n}
\newcommand{\tens}[1]{\bm{\mathsfit{#1}}}
\def\tA{{\tens{A}}}
\def\tB{{\tens{B}}}
\def\tC{{\tens{C}}}
\def\tD{{\tens{D}}}
\def\tE{{\tens{E}}}
\def\tF{{\tens{F}}}
\def\tG{{\tens{G}}}
\def\tH{{\tens{H}}}
\def\tI{{\tens{I}}}
\def\tJ{{\tens{J}}}
\def\tK{{\tens{K}}}
\def\tL{{\tens{L}}}
\def\tM{{\tens{M}}}
\def\tN{{\tens{N}}}
\def\tO{{\tens{O}}}
\def\tP{{\tens{P}}}
\def\tQ{{\tens{Q}}}
\def\tR{{\tens{R}}}
\def\tS{{\tens{S}}}
\def\tT{{\tens{T}}}
\def\tU{{\tens{U}}}
\def\tV{{\tens{V}}}
\def\tW{{\tens{W}}}
\def\tX{{\tens{X}}}
\def\tY{{\tens{Y}}}
\def\tZ{{\tens{Z}}}


% Graph
\def\gA{{\mathcal{A}}}
\def\gB{{\mathcal{B}}}
\def\gC{{\mathcal{C}}}
\def\gD{{\mathcal{D}}}
\def\gE{{\mathcal{E}}}
\def\gF{{\mathcal{F}}}
\def\gG{{\mathcal{G}}}
\def\gH{{\mathcal{H}}}
\def\gI{{\mathcal{I}}}
\def\gJ{{\mathcal{J}}}
\def\gK{{\mathcal{K}}}
\def\gL{{\mathcal{L}}}
\def\gM{{\mathcal{M}}}
\def\gN{{\mathcal{N}}}
\def\gO{{\mathcal{O}}}
\def\gP{{\mathcal{P}}}
\def\gQ{{\mathcal{Q}}}
\def\gR{{\mathcal{R}}}
\def\gS{{\mathcal{S}}}
\def\gT{{\mathcal{T}}}
\def\gU{{\mathcal{U}}}
\def\gV{{\mathcal{V}}}
\def\gW{{\mathcal{W}}}
\def\gX{{\mathcal{X}}}
\def\gY{{\mathcal{Y}}}
\def\gZ{{\mathcal{Z}}}

% Sets
\def\sA{{\mathbb{A}}}
\def\sB{{\mathbb{B}}}
\def\sC{{\mathbb{C}}}
\def\sD{{\mathbb{D}}}
% Don't use a set called E, because this would be the same as our symbol
% for expectation.
\def\sF{{\mathbb{F}}}
\def\sG{{\mathbb{G}}}
\def\sH{{\mathbb{H}}}
\def\sI{{\mathbb{I}}}
\def\sJ{{\mathbb{J}}}
\def\sK{{\mathbb{K}}}
\def\sL{{\mathbb{L}}}
\def\sM{{\mathbb{M}}}
\def\sN{{\mathbb{N}}}
\def\sO{{\mathbb{O}}}
\def\sP{{\mathbb{P}}}
\def\sQ{{\mathbb{Q}}}
\def\sR{{\mathbb{R}}}
\def\sS{{\mathbb{S}}}
\def\sT{{\mathbb{T}}}
\def\sU{{\mathbb{U}}}
\def\sV{{\mathbb{V}}}
\def\sW{{\mathbb{W}}}
\def\sX{{\mathbb{X}}}
\def\sY{{\mathbb{Y}}}
\def\sZ{{\mathbb{Z}}}

% Entries of a matrix
\def\emLambda{{\Lambda}}
\def\emA{{A}}
\def\emB{{B}}
\def\emC{{C}}
\def\emD{{D}}
\def\emE{{E}}
\def\emF{{F}}
\def\emG{{G}}
\def\emH{{H}}
\def\emI{{I}}
\def\emJ{{J}}
\def\emK{{K}}
\def\emL{{L}}
\def\emM{{M}}
\def\emN{{N}}
\def\emO{{O}}
\def\emP{{P}}
\def\emQ{{Q}}
\def\emR{{R}}
\def\emS{{S}}
\def\emT{{T}}
\def\emU{{U}}
\def\emV{{V}}
\def\emW{{W}}
\def\emX{{X}}
\def\emY{{Y}}
\def\emZ{{Z}}
\def\emSigma{{\Sigma}}

% entries of a tensor
% Same font as tensor, without \bm wrapper
\newcommand{\etens}[1]{\mathsfit{#1}}
\def\etLambda{{\etens{\Lambda}}}
\def\etA{{\etens{A}}}
\def\etB{{\etens{B}}}
\def\etC{{\etens{C}}}
\def\etD{{\etens{D}}}
\def\etE{{\etens{E}}}
\def\etF{{\etens{F}}}
\def\etG{{\etens{G}}}
\def\etH{{\etens{H}}}
\def\etI{{\etens{I}}}
\def\etJ{{\etens{J}}}
\def\etK{{\etens{K}}}
\def\etL{{\etens{L}}}
\def\etM{{\etens{M}}}
\def\etN{{\etens{N}}}
\def\etO{{\etens{O}}}
\def\etP{{\etens{P}}}
\def\etQ{{\etens{Q}}}
\def\etR{{\etens{R}}}
\def\etS{{\etens{S}}}
\def\etT{{\etens{T}}}
\def\etU{{\etens{U}}}
\def\etV{{\etens{V}}}
\def\etW{{\etens{W}}}
\def\etX{{\etens{X}}}
\def\etY{{\etens{Y}}}
\def\etZ{{\etens{Z}}}

% The true underlying data generating distribution
\newcommand{\pdata}{p_{\rm{data}}}
% The empirical distribution defined by the training set
\newcommand{\ptrain}{\hat{p}_{\rm{data}}}
\newcommand{\Ptrain}{\hat{P}_{\rm{data}}}
% The model distribution
\newcommand{\pmodel}{p_{\rm{model}}}
\newcommand{\Pmodel}{P_{\rm{model}}}
\newcommand{\ptildemodel}{\tilde{p}_{\rm{model}}}
% Stochastic autoencoder distributions
\newcommand{\pencode}{p_{\rm{encoder}}}
\newcommand{\pdecode}{p_{\rm{decoder}}}
\newcommand{\precons}{p_{\rm{reconstruct}}}

\newcommand{\laplace}{\mathrm{Laplace}} % Laplace distribution

\newcommand{\E}{\mathbb{E}}
\newcommand{\Ls}{\mathcal{L}}
\newcommand{\R}{\mathbb{R}}
\newcommand{\emp}{\tilde{p}}
\newcommand{\lr}{\alpha}
\newcommand{\reg}{\lambda}
\newcommand{\rect}{\mathrm{rectifier}}
\newcommand{\softmax}{\mathrm{softmax}}
\newcommand{\sigmoid}{\sigma}
\newcommand{\softplus}{\zeta}
\newcommand{\KL}{D_{\mathrm{KL}}}
\newcommand{\Var}{\mathrm{Var}}
\newcommand{\standarderror}{\mathrm{SE}}
\newcommand{\Cov}{\mathrm{Cov}}
% Wolfram Mathworld says $L^2$ is for function spaces and $\ell^2$ is for vectors
% But then they seem to use $L^2$ for vectors throughout the site, and so does
% wikipedia.
\newcommand{\normlzero}{L^0}
\newcommand{\normlone}{L^1}
\newcommand{\normltwo}{L^2}
\newcommand{\normlp}{L^p}
\newcommand{\normmax}{L^\infty}

\newcommand{\parents}{Pa} % See usage in notation.tex. Chosen to match Daphne's book.

\DeclareMathOperator*{\argmax}{arg\,max}
\DeclareMathOperator*{\argmin}{arg\,min}

\DeclareMathOperator{\sign}{sign}
\DeclareMathOperator{\Tr}{Tr}
\let\ab\allowbreak


==> review.tex <==
\pdfoutput=1
\section{CVPR2020 reviews and \textcolor{blue}{author response}}

We first mention that we have not submitted a rebuttal for the CVPR reviews as we felt the review quality was not great. We instead decided to submit again to the NTIRE workshop as the reviewers for a more focused workshop relevant to our paper would have a better understanding and give a more constructive review. We put our (unsubmitted) rebuttal below for each review. 


\subsection{Reviwer1}
1. [Summary] In 3-5 sentences, describe the key ideas, experiments, and their significance. 
This paper proposes a GAN2GAN (Generated-Artificial-Noise to Generated-Artificial-Noise) method for blind image denoising with the assumption of 
zero-mean, additive and independent noise. The main idea is to sythesize noisy image pair via GAN and then train the denoising network via N2N method.
Experiments validated the effectiveness of the proposed method over N2N and BM3D. \\
2. [Strengths] What are the strengths of the paper? Clearly explain why these aspects of the paper are valuable. \\
This paper is well-organized and well-written.
The noise assumption is rather clear.
The details are very clear.  \\
3. [Weaknesses] What are the weaknesses of the paper? Clearly explain why these aspects of the paper are weak. Please make the comments very concrete based on facts (e.g. list relevant citations if you feel the ideas are not novel). \\
1) The role of $g_3$ which maps clean image to noisy image is questionable. Actually, $g_3$ is a one-to-many problem, it is difficult to map a clean image to a noisy one which has low MSE to the original noisy image. \\
\textcolor{blue}{[Author response]: We agree that obtaining $g_3$ is a one-to-many problem, hence, it is difficult to train $g_3$. However, we experimentally showed that the CycleLoss with $g_3$ helps to increase PSNR of $g_2$ in Fig 3(c)[in the manuscript], and we want to argue that many kinds of loss functions similar to CycleLoss are generally used in many papers to reconstruct a clean source.} \\
2) The noise is assumed to be independent to the clean image, is it also independent identically distributed? If yes, then how to guarantee $g_{1}(r)$ is identically distributed? \\
\textcolor{blue}{[Author response]: After the noise patch extraction, we can get a set of noise patches and then we train $g_{1}$ with these patches. We did not add any kinds of constraints to make $g_{1}(r)$ independent identically distributed(iid), however, we checked that, from Tab1, we could get competitive results by using $g_{1}(r)$, and it means that our $g_{1}(r)$ learns and generates iid noise which is similar with a noise in the noisy images. From these results, we think that we experimentally showed our $g_{1}(r)$ can generates and learn iid noise successfully.}
3) The proposed method needs to extract the noise from smooth region. However, to my knowledge, the BSD400 image does not contain rich smooth regions. Does it inflence the proposed method? \\
\textcolor{blue}{[Author response]: If there is a limited number of smooth regions, we can control the smoothness of extracted patches by controlling $\lambda$, and we can still apply our method. However, as you expected, the denoising results will degrade in this case. In our opinion, we think that this comment is too harsh because the cost of collecting many noisy images is much cheaper than the cost of collecting paired clean images. Therefore, if we are able to get a large size of noisy images (larger than BSD400), the number of smooth patches also increase so our method will show the better result.}\\
4. [Overall rating] Paper rating (pre-rebuttal) \\ 
Borderline \\
5. [Justification of rating] Please explain how the strengths and weaknesses aforementioned were weighed in for the rating. Please also mention what you expect to see from the rebuttal that may change your rating. \\
See the Weaknesses. \\
% 11. Final rating \\
% Weak reject \\
% 12. Explanation of final rating. Describe the rationale for your final rating, including notes based on the rebuttal, discussion, and other reviews. \\
% The role of g1(r) to generate noisy images does not make sense. \\

\subsection{Reviwer2}
1. [Summary] In 3-5 sentences, describe the key ideas, experiments, and their significance. \\
In this paper, the authors propose to synthesize noisy image pairs by a generative model, and then train a denoiser with those synthesized pairs, as in the N2N training. The model could be trained based on a single image. The results outperforms Noise2Void for the same setting, and approaches the performance of N2N which has more information. \\
2. [Strengths] What are the strengths of the paper? Clearly explain why these aspects of the paper are valuable. \\
1) This paper proposes a novel way to denoise an image which makes the training even possible from a single image. \\
3. [Weaknesses] What are the weaknesses of the paper? Clearly explain why these aspects of the paper are weak. Please make the comments very concrete based on facts (e.g. list relevant citations if you feel the ideas are not novel). \\
1) For real image denoising, the experiments are only performed on microscopy image datasets, which is not a commonly used real image testing dataset. For sufficient verification of the proposed method, it is suggested to try the public real image denoising dataset RNI15, DND, SIDD, etc.
\textcolor{blue}{[Author response]: Our method essentially consider a source independent noise so our method is not able to directly apply to the real noise dataset you mentioned, which have source-dependent noise. However, we are able to apply our method to the microscopy dataset because, in this dataset, there are small source dependent noise area than other real noise dataset(this analysis is in Supplementary). Extending our GAN2GAN framework for the source-dependent noise is the topic for our future work.}\\
2) As shown in Table 1, although training from single image is possible, the PSNR/SSIM performance is not satisfactory (around 2dB less) compared with training from a full dataset. As such, the title sounds true but over-claimed.
\textcolor{blue}{[Author response]: There is no results that our results showed around 2dB less than training a full dataset. Also, we think that, compared with  N2V which also consider training from single noisy images, we achieve much closer results to training with a full dataset. Moreover, as we mentioned in the Introduction, there are applications in which no clean images are available for supervised training, and our methodology is targeted to such harsh settings.}\\
4. [Overall rating] Paper rating (pre-rebuttal) \\
Weak reject \\
5. [Justification of rating] Please explain how the strengths and weaknesses aforementioned were weighed in for the rating. Please also mention what you expect to see from the rebuttal that may change your rating. \\
The most important factors for my overall recommendation are the insufficient experiments and over-claim of single image training of the paper, as described in [Weaknesses]. I think the current form is not ready for the publication. \\
6. [Detailed comments] Additional comments regarding the paper (e.g. typos, any suggestions to make the submission stronger). \\
1) The Lena image in Figure 1 is misleading. In this paper, it means a patch of an image, however, the Lena image frequently used in research papers means a full image. Please change to image patches accordingly.
2) Please refer to the weaknesses of the paper. Please address my concerns in the rebuttal document. \\
% 11. Final rating \\
% Weak reject \\
% 12. Explanation of final rating. Describe the rationale for your final rating, including notes based on the rebuttal, discussion, and other reviews. \\
% The author did not provide feedback. I will keep my original rating as weak reject. \\

\subsection{Reviwer3}
1. [Summary] In 3-5 sentences, describe the key ideas, experiments, and their significance. \\
This paper aims to tackle a blind image denoising problem with single distinct noisy images. It proposes GAN2GAN to learn a generative model to synthesize noisy image pairs and then perform denoising by N2N. Experimental results demonstrate the effectiveness of the proposed method. \\
2. [Strengths] What are the strengths of the paper? Clearly explain why these aspects of the paper are valuable. \\
1) The proposed method combines data augmentation through GAN and the unsupervised Noise2Noise method for blind image denoising with single noisy image. \\
2) The proposed method achieves favorable denoising performance. \\
3. [Weaknesses] What are the weaknesses of the paper? Clearly explain why these aspects of the paper are weak. Please make the comments very concrete based on facts (e.g. list relevant citations if you feel the ideas are not novel). \\
1) In this paper, the authors assume that the noise should be zero-mean and additive and independent of the clean image, which limits the practicability and generalization on the real-world photographs since that the noise in real is more complicated. \\
\textcolor{blue}{[Author response]: We agree with your opinion and our future work is extending our GAN2GAN framework to the real-world photographs denoising (without clean target images). Our proposed GAN2GAN is indeed in the setting you mentioned, but it still achieves much better results than N2V, which is considered to be the state-of-the-art for the same setting. }\\
2) The proposed method is more like an ensemble of existing works, i.e., GCBD [5], W-GAN [1] and N2N [13], which limits the novelty and contribution of this work. \\
\textcolor{blue}{[Author response]: We do not think that our method is just an ensemble of existing works. It is true that we cited the ideas of the papers you mentioned papers, but through this, we proposed a more improved noise patch extraction method, a new structure for training GAN using only noisy images, and the ideas of iterative N2N. By using these newly proposed idea, we showed that training a NN-based denoiser is possible with single noisy images which was not overcome in the referenced papers.}\\
3) In the training of the generative model, $f_{w_1}$ is a discriminator to distinguish the real noisy image from the fake noisy image. However, the discriminator in WGAN focus more on the image content. Please provide more analysis on the effeteness of LZ . \\
\textcolor{blue}{[Author response]: We don't agree that WGAN focus more on the image content. This is because, if it is true, our $f_{w_1}$ cannot be trained with noise patches which contain information only on the noise distribution not the image content. We believe that WGAN makes the true distribution and the fake distribution close, and as a result, our $g_{\theta_1}$ and $g_{\theta_2}$ are successfully trained and showed a competitive result in the process of G2G iterative training.}\\
4) $Z^1$ , $Z^2$ is constructed by the generated fake clean image $g_{\theta_2}$. It needs to be clarified that how to make sure $g_{\theta_2}$ is a clean image. If not, the noise in $Z^1$ , $Z^2$ is not independent. \\
\textcolor{blue}{[Author response]: $Z^1$ is generated by $Z^1 = g_{\theta_1}(Z) + g_{\theta_2}(r_1)$ and $Z^2$ is generated by $Z^2 = g_{\theta_1}(Z) + g_{\theta_2}(r_2)$. Therefore, $g_{\theta_2}(r_1)$ and $g_{\theta_2}(r_1)$ are solely independent with $g_{\theta_2}$ so $Z^1$ and $Z^2$ can be independent.}\\
5) It is suggested to provide some visualization experiments on the real-world photographs, such as DND. \\
\textcolor{blue}{[Author response]: Applying to the real-work photographs is our future work.}\\
4. [Overall rating] Paper rating (pre-rebuttal) \\
Weak reject \\
5. [Justification of rating] Please explain how the strengths and weaknesses aforementioned were weighed in for the rating. Please also mention what you expect to see from the rebuttal that may change your rating. \\
Lacking novelty and contributions are the main concern of this work, even though they achieve promising results. Details can be found in the Weaknesses. \\
% 11. Final rating \\
% Weak reject \\
% 12. Explanation of final rating. Describe the rationale for your final rating, including notes based on the rebuttal, discussion, and other reviews. \\
% I agree with Reviewer 1. Furthermore, the authors did not provide the rebuttal. I will keep the initial rating. \\


\clearpage
